Resource Allocation Game on Social Networks: Best Response Dynamics and Convergence

The decisions that human beings make to allocate time has significant bearing on economic output and to the sustenance of social networks. The time allocation problem motivates our formal analysis of the resource allocation game, where agents on a social network, who have asymmetric, private interaction preferences, make decisions on how to allocate time, a bounded endowment, over their neighbors. Unlike the well-known opinion formation game on a social network, our game appears not to be a potential game, and the Best-Response dynamics is non-differentiable making the analysis of Best-Response dynamics non-trivial. In our game, we consider two types of player behavior, namely optimistic or pessimistic, based on how they use their time endowment over their neighbors. To analyze Best-Response dynamics, we circumvent the problem of the game not being a potential game, through the lens of a novel two-level potential function approach. We show that the Best-Response dynamics converges point-wise to a Nash Equilibrium when players are all: optimistic; pessimistic; a mix of both types. Finally, we show that the Nash Equilibrium set is non-convex but connected, and Price of Anarchy is unbounded while Price of Stability is one. Extensive simulations over a stylized grid reveals that the distribution of quality of the convergence points is unimodal-we conjecture that presence of unimodality is tied to the connectedness of Nash Equilibrium.

==> technicalcontributions.tex <==
% !TEX Root=paper.tex

\subsection{Our Technical Contributions}
\label{sub:Technical Contributions}

We study the {\em resource allocation} game on (social) network $G=(V,E)$ where each node $i\in V$ is a rational player (agent) with finite time endowment, say $\beta_i$. A player $i$ gains utility by spending time with her network neighbors $\mathcal{N}_i$ and wants to distribute her time endowment strategically. Each player $i$ has \textit{private} preferences $w_{ij}$ over her neighbors $j \in \mathcal{N}_i$, where $\sum_{j \in \mathcal{N}_i} w_{ij} = 1$. In other words, an agent obtains utility by spending time communicating with her network neighbors. In general, we consider the asymmetric case where $w_{ij} \neq w_{ji}$, implying that $i$ and $j$ may differ in their preferences to interact with each other.

A pair of players who are neighbors i.e. $(i,j)\in E$, interact when both agree to do so. Thus, if $f_{ij}$ is the (time) interaction frequency ``proposed'' by $i$ to $j$, and $f_{ji}$ by $j$ to $i$, then the pair will agree to $f^*_{i,j} = \min\{f_{ij},f_{ji}\}$. The total utility of agent $i$ is:
\[
 \sum_{j\in \mathcal{N}_i} w_{ij} u_{ij}(f^*_{ij}),
\]
where $u_{ij}$'s are non-negative increasing concave functions which capture decreasing marginal returns.

% If the endowment is the same across the network (e.g. everyone has twenty four hours in a day to distribute), then since a pair interacts with a mutually agreed upon frequency $f_{i,j}^*$, we let $u_{ij}=u_{ji}$ for all $(i,j)\in E$. Since the weights capture preference asymmetry, we $i$ and $j$ will still derive different utilities.
%Whether a player is willing allocate her ``left over'' resource to neighbors in anticipation of response, we classify players into optimistic and pessimistic. The former may allocate the latter does not.
% \rnote{should we talk about optimistic and pessimistic players?}

Our main contribution is in the convergence analysis of {\em best-response} dynamics for resource allocation games. In each round, a chosen player (in some arbitrary sequence) plays her utility maximizing (best-response) strategy given the proposals of her network neighbors. We know that best-response dynamics may not converge in general, but does converge in potential games~\cite{monderer:96}. What makes our problem interesting and challenging is that preference asymmetry (i.e. $w_{ij} \neq w_{ji}$ in general) implies that \textit{our game is not in general a potential game}.

We consider a natural subclass where agents have inherent social order (e.g.  a management hierarchy). Then, we let the preference weight $w_{ij}$ be proportional to the global social rank; we call such a weighting mechanism a {\em global ranking weight system}. Our first result (see Section \ref{sec:conv:seq:gr}):

\begin{theorem}[Informal]
 The resource allocation game with global ranking weight system is a weighted potential game. As a consequence, the best-response dynamics in these games converges to a Nash equilibrium.
\end{theorem}

Though the general resource allocation game is not a potential game, we show a key result in Section~\ref{sec:conv:seq:gen}:

\begin{theorem}[Informal]
 Best response dynamics converges to a Nash equilibrium in general resource allocation games with asymmetric preferences.
\end{theorem}

Our method of proof is akin to the construction of a ``two-level'' potential-like function using the unused total time of a specific class of players. We show that the outer function is monotonically decreasing, and when the outer function is fixed, the inner function decreases.

Next we consider the {\em simultaneous play} variant of the best-response dynamics of the general resource constrained game, where all players simultaneously update their strategies in every round. We show the existence of a cycle, through a stylized example. Note that potential games \cite{monderer:96} {\em e.g.,} battle of the sexes may also exhibit cycles in simultaneous play.

Having shown that best response dynamics in the general game converges to a Nash Equilibria, we focus on \textit{characterization}, \textit{quality} (social-welfare) and \textit{stability} of the equilibria. We show that the Price-of-Anarchy (PoA) is unbounded while Price-of-Stability (PoS) is one. Furthermore, the set of Nash Equilibrium set is convex under certain behavioral assumptions and connected in general. Experiments on a stylized grid show that best response dynamics converge to equilibria with high social-welfare (see Section \ref{sec:exper}). Our result on stability is that even the {\em best-quality} Nash equilibria need not be stable. That is, the best-response dynamics given an $\epsilon$-ball perturbation of the best-quality Nash Equilibria may move the network out of the ball. We note that for the network to move out of the ball, the order in which players update seems to be crucial. Since the order of the moves does not affect convergence, the best response dynamics may still converge to a high quality Nash Equilibria. Finally, it will be interesting to analyze the convergence quality through the {\em average-price-of-anarchy} \cite{PP16}, a question that we leave open.

% Although the convergence result holds, independent of the order of the moves. This still does not rule out convergence to NE with good social-welfare, and it would be really interesting to analyze this through the {\em average-price-of-anarchy} \cite{PP} which we leave open.

% One way to approach this problem formally is through stability analysis of the high-quality convergence points.

% Through an example we show that even the {\em best-quality} Nash equilibria need not be stable \cite{}, {\em i.e,} starting within an $\epsilon$-ball around it the dynamics may move outside the ball. We note that for this to happen, the order in which players update seems crucial. Although the convergence results hold independent of the order. This still does not rule out convergence to NE with good social-welfare, and it would be really to analyze this through the {\em average-price-of-anarchy} \cite{PP} which we leave open.

